PsyChat: A Client-Centric Dialogue System for Mental Health Support

Dialogue systems are increasingly integrated into mental health support to help clients facilitate exploration, gain insight, take action, and ultimately heal themselves. A practical and user-friendly dialogue system should be client-centric, focusing on the client's behaviors. However, existing dialogue systems publicly available for mental health support often concentrate solely on the counselor's strategies rather than the behaviors expressed by clients. This can lead to unreasonable or inappropriate counseling strategies and corresponding responses generated by the dialogue system. To address this issue, we propose PsyChat, a client-centric dialogue system that provides psychological support through online chat. The client-centric dialogue system comprises five modules: client behavior recognition, counselor strategy selection, input packer, response generator, and response selection. Both automatic and human evaluations demonstrate the effectiveness and practicality of our proposed dialogue system for real-life mental health support. Furthermore, the case study demonstrates that the dialogue system can predict the client's behaviors, select appropriate counselor strategies, and generate accurate and suitable responses.

==> 7-bib.tex <==
\begin{thebibliography}{00}
\bibitem{MentalHealth} M. Prince, V. Patel, S. Saxena, M. Maj, J. Maselko, M. R. Phillips, and A. Rahman. ``No health without mental health." The lancet 370, no. 9590 (2007): 859-877.

\bibitem{HelpingSkills2009} C. E. Hill. ``Helping skills: Facilitating, exploration, insight, and action." American Psychological Association, 2009.


\bibitem{psyqa2021sun} H. Sun, Z. Lin, C. Zheng, S. Liu and M. Huang. ``Psyqa: A chinese dataset for generating long counseling text for mental health support." arXiv preprint arXiv:2106.01702 (2021).

\bibitem{esconv2021liu} S. Liu, C. Zheng, O. Demasi, S. Sabour, Y. Li, Z. Yu, Y. Jiang and M. Huang. ``Towards emotional support dialog systems." arXiv preprint arXiv:2106.01144 (2021).

\bibitem{augesc2022zheng} C. Zheng, S. Sabour, J. Wen, Z. Zhang and M. Huang. ``Augesc: Large-scale data augmentation for emotional support conversation with pre-trained language models." arXiv preprint arXiv:2202.13047 (2022).

\bibitem{smile2023qiu} H. Qiu, H. He, S. Zhang, A. Li, and Z. Lan. ``SMILE: Single-turn to Multi-turn Inclusive Language Expansion via ChatGPT for Mental Health Support." arXiv preprint arXiv:2305.00450 (2023).

\bibitem{soulchat2023chen} Y. Chen, X. Xing, J. Lin, H. Zheng, Z. Wang, Q. Liu and X. Xu. ``SoulChat: Improving LLMs' Empathy, Listening, and Comfort Abilities through Fine-tuning with Multi-turn Empathy Conversations." arXiv preprint arXiv:2311.00273 (2023).

\bibitem{chatcounselor2023liu} J. M. Liu, D. Li, H. Cao, T. Ren, Z. Liao and J. Wu. ``Chatcounselor: A large language models for mental health support." arXiv preprint arXiv:2309.15461 (2023).

\bibitem{client2023li} A. Li, L. Ma, Y. Mei, H. He, S. Zhang, H. Qiu, and Z. Lan, 2023. ``Understanding Client Reactions in Online Mental Health Counseling." In Proceedings of ACL, pages 10358–10376, Toronto, Canada.

\bibitem{ChatGLM} A. Zeng, X. Liu, Z. Du, Z.Wang, H. Lai, M. Ding, Z. Yang, Y. Xu, W. Zheng, X. Xia and W.L. Tam. ``Glm-130b: An open bilingual pre-trained model." arXiv preprint arXiv:2210.02414 (2022).

\bibitem{RoBERTa} Y. Cui, W.g Che, T. Liu, B. Qin, S. Wang, and G. Hu. 2020. ``Revisiting Pre-Trained Models for Chinese Natural Language Processing." In Findings of the Association for Computational Linguistics: EMNLP 2020, pages 657–668, Online. Association for Computational Linguistics.



\bibitem{hu2021lora} E. J. Hu, Y. Shen, P. Wallis, Z. Allen-Zhu, Y. Li, S. Wang, L. Wang, and W. Chen. ``Lora: Low-rank adaptation of large language models." in arXiv, preprint arXiv:2106.09685.

\bibitem{Perplexity} F. Jelinek, R. L. Mercer, L. R. Bahl, and J. K. Baker. ``Perplexity—a measure of the difficulty of speech recognition tasks." The Journal of the Acoustical Society of America 62, no. S1 (1977): S63-S63.

\bibitem{Meteor} S. Banerjee and A. Lavie. ``METEOR: An automatic metric for MT evaluation with improved correlation with human judgments." In Proceedings of the ACL workshop, pp. 65-72. 2005.

\bibitem{Bleu} K. Papineni, S. Roukos, T. Ward, and W. Zhu. ``Bleu: a method for automatic evaluation of machine translation." In Proceedings of the 40th annual meeting of the Association for Computational Linguistics, pp. 311-318. 2002.

\bibitem{Rouge} C. Lin. ``Rouge: A package for automatic evaluation of summaries." In Text summarization branches out, pp. 74-81. 2004.


\bibitem{Diversity} J. Li, M. Galley, C. Brockett, J. Gao, and B. Dolan. ``A diversity-promoting objective function for neural conversation models." arXiv preprint arXiv:1510.03055 (2015).




\end{thebibliography}
